FlowZero: Zero-Shot Text-to-Video Synthesis with LLM-Driven Dynamic Scene Syntax

Text-to-video (T2V) generation is a rapidly growing research area that aims to translate the scenes, objects, and actions within complex video text into a sequence of coherent visual frames. We present FlowZero, a novel framework that combines Large Language Models (LLMs) with image diffusion models to generate temporally-coherent videos. FlowZero uses LLMs to understand complex spatio-temporal dynamics from text, where LLMs can generate a comprehensive dynamic scene syntax (DSS) containing scene descriptions, object layouts, and background motion patterns. These elements in DSS are then used to guide the image diffusion model for video generation with smooth object motions and frame-to-frame coherence. Moreover, FlowZero incorporates an iterative self-refinement process, enhancing the alignment between the spatio-temporal layouts and the textual prompts for the videos. To enhance global coherence, we propose enriching the initial noise of each frame with motion dynamics to control the background movement and camera motion adaptively. By using spatio-temporal syntaxes to guide the diffusion process, FlowZero achieves improvement in zero-shot video synthesis, generating coherent videos with vivid motion.

==> sec/1_intro_back.tex <==
\section{Introduction}
\label{sec:intro}

In the field of AI-generated content, there has been growing interest in expanding the generative capabilities of pre-trained text-to-image (T2I) models to text-to-video (T2V) generation~\cite{animatediff,cogvideo,direct2v,free-bloom,ImagenVideo,MagicVideo,t2vz,videofusion,makeavideo}.
Recent studies have introduced zero-shot T2V~\cite{t2vz, free-bloom, direct2v}, which aims to adapt image diffusion models for video generation without additional training. These methods utilize the capabilities of image diffusion models, originally trained on static images, to generate frame sequences from video text prompts. 
However, generating coherent dynamic visual scenes in videos remains challenging due to the succinct and abstract nature of video text prompts.

To address this, recent research~\cite{free-bloom,direct2v} proposes utilizing Large Language Models (LLMs) to breakdown video text into frame-level descriptions.
These descriptions are crafted to represent each moment or event within the video, guiding image diffusion models to generate semantic-coherent videos.
However, these frame-level descriptions only capture the basic temporal semantics of video prompts, lacking in detailed spatio-temporal information necessary for ensuring smooth object motion and consistent frame-to-frame coherence in videos.

Recent advancements in text-to-image generation~\cite{layoutgpt, visorgpt, controlgpt} 
have shown the effectiveness of LLMs in planning spatial arrangements for images.
These studies demonstrate that LLMs can generate accurate spatial layouts for foreground objects from text prompts, guiding diffusion models to generate images with coherent
spatial relationships.
These capabilities indicate a potential for LLMs to understand complex video prompts and generate fine-grained spatio-temporal layouts to guide video synthesis.
However, generating spatio-temporal layouts for videos is more intricate than for static images. This is because it necessitates the LLMs to comprehend and illustrate how objects move and transform over time.
Additionally, representing global background movement to depict camera motion is crucial for immersive video generation~\cite{camera1,camera2}, which further complicates the video generation.

In this paper, we introduce \textbf{\textit{FlowZero}}, a novel framework that integrates LLMs with image diffusion models to generate temporally-coherent videos from text prompts. 
FlowZero utilizes LLMs for comprehensive analysis and translating the video text prompt into a proposed structured Dynamic Scene Syntax~(DSS). Unlike previous methods that only basic semantic descriptions, the DSS contains scene descriptions, layouts for foreground objects, and background motion patterns.
Foreground layouts contain a series of bounding boxes that define each frame's spatial arrangement and track changes in the positions and sizes of objects. This ensures that the object motion and transformation align with the textual prompt.
Additionally, FlowZero incorporates an iterative self-refinement process. This process effectively enhances the correlation between the generated layouts and the textual descriptions, specifically addressing inaccuracies such as spatial and temporal errors. In the self-refinement process, the generated layouts are continuously compared and adjusted against the text through a feedback loop, ensuring a high fidelity and coherence of the spatio-temporal layouts. 

FlowZero prompts LLMs to predict background motion patterns to enhance temporal coherence and consistency, which can be used to control global scenes and camera motion in video frames.
For instance, consider a text that describes a horse running from right to left, as shown in the middle example of Figure~\textcolor{red}{1}. The LLMs predict a corresponding camera motion, making the background move from left to right, enhancing the video's immersiveness~\cite{camera1,camera2}.
The background motion pattern includes specific directions and speeds to indicate the background motion pattern.
We shift the initial noise for each frame according to the predicted direction and speed, resulting in a more temporal-smooth synthesis.

FlowZero achieves a significant advancement in zero-shot text-to-video synthesis, utilizing the spatio-temporal planning ability of LLMs to generate detailed frame-by-frame syntax to enhance text-to-video generation. The fusion of these technologies within the FlowZero framework enables the generation of temporally-coherent, visually appealing videos directly from textual prompts.

Our contributions are summaries as follows:

\begin{itemize}
    \item We introduce FlowZero, which uses LLMs to convert text into Dynamic Scene Syntax, leading to accurate frame-by-frame video instructions. The framework's iterative self-refinement process ensures better alignment of spatio-temporal layouts with text prompts, enhancing video synthesis consistency and fidelity.

    \item FlowZero improves the global coherence of videos with controlled background motion, achieved through motion-guided noise shifting. This enhances the realism of the scene and camera movements.

\item Through extensive experiments and evaluations, we demonstrate FlowZero's capability to generate temporally coherent videos that accurately depict complex motions and transformations as described in textual prompts.

\item 
\end{itemize}

\begin{figure*}[h]
\centering
   \setlength{\abovecaptionskip}{0.5cm}
   \includegraphics[scale = 0.68]{images/framework_all.pdf}
     \caption{
     \textbf{Overview of FlowZero.} Our pipeline consists of two interconnected stages: (1) Syntax Generation, (2) Video Synthesis. In the Syntax generation stage, the LLM~(\ie, GPT4) is prompted to generate serial frame-by-frame syntax, including scene descriptions, foreground layouts, and background motion direction and scale. We employ an iterative self-refinement process to improve the generated spatio-temporal layouts. This includes incorporating a feedback loop where the LLM autonomously verifies and corrects the spatial and temporal errors of the initial layouts.
     In the Video synthesis stage, we first utilize background motions to guide the shifting of the initial noise for each frame~(MNS). Then, a U-Net with cross-attention, gated attention, and cross-frame attention is used to obtain the coherent video frames.
     }
   \label{fig:pipeline}
\end{figure*}
